In Situ AI Prototyping: Infusing Multimodal Prompts into Mobile Settings with MobileMaker

Recent advances in multimodal large language models (LLMs) have made it easier to rapidly prototype AI-powered features, especially for mobile use cases. However, gathering early, mobile-situated user feedback on these AI prototypes remains challenging. The broad scope and flexibility of LLMs means that, for a given use-case-specific prototype, there is a crucial need to understand the wide range of in-the-wild input users are likely to provide and their in-context expectations for the AI's behavior. To explore the concept of in situ AI prototyping and testing, we created MobileMaker: a platform that enables designers to rapidly create and test mobile AI prototypes directly on devices. This tool also enables testers to make on-device, in-the-field revisions of prototypes using natural language. In an exploratory study with 16 participants, we explored how user feedback on prototypes created with MobileMaker compares to that of existing prototyping tools (e.g., Figma, prompt editors). Our findings suggest that MobileMaker prototypes enabled more serendipitous discovery of: model input edge cases, discrepancies between AI's and user's in-context interpretation of the task, and contextual signals missed by the AI. Furthermore, we learned that while the ability to make in-the-wild revisions led users to feel more fulfilled as active participants in the design process, it might also constrain their feedback to the subset of changes perceived as more actionable or implementable by the prototyping tool.

==> figures/figure-4.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{assets/images/figure-4/agile-row.png}
\vspace{-3mm}
\caption{Traditional (left) vs. in situ (right) prototyping cycles.
% Traditionally, designers, developers, user researchers, and end users have distinct roles; in situ prototyping allows these roles to blur and broaden participation in AI development.
}
\label{fig:agile}
\vspace{-4mm}
\end{figure}
